Codes on any Cayley Graph have an Interactive Oracle Proof of Proximity

Interactive Oracle Proofs of Proximity (IOPP) are at the heart of code-based SNARKs, a family of zeroknowledge protocols. The first and most famous one is the FRI protocol [BBHR18a], that efficiently tests proximity to Reed-Solomon codes. This paper generalizes the flowering IOPP introduced in [DMR25] for some specific (2, n)-regular Tanner codes to a much broader variety of codes: any code with symbols indexed on the edges of a Cayley graph. The flowering protocol of [DMR25] had a soundness parameter much lower than the FRI protocol [BCI + 23], and complexity parameters that could compete with the FRI [BBHR18a]. The lower soundness and the absence of restriction on the base field may lead to other practical speedups, however the codes considered in [DMR25] have an o(1) minimum distance. The generalization proposed in this paper preserves the soundness parameter with a slight decrease of the complexity parameters, while allowing being applied on codes with constant rate and constant minimum distance thanks to the good expansion properties of some families of Cayley graphs.

==> src/cayley-graphs.tex <==
\section{Cutting Cayley Graphs}


\input{src/cayley-cut}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../CANS"
%%% End:


==> src/conclusion.tex <==
\section{Conclusion}

This paper generalized the IOPP for codes on $(2,n)$-regular Tanner graphs introduced in \cite{DMR25} that was only applied on codes with $o(1)$ minimum distance to any $(2,n)$-regular Tanner graph built as a Cayley graph.
This generalization allows to use Cayley graphs with good expansion, yielding codes with constant rate and minimum distance.
The great soundness parameter from~\cite{DMR25} compared to the FRI protocol~\cite{BCIKS23} is thus preserved, even if the complexity becomes slightly higher, while now allowing the use of codes with constant rate and constant minimum distance.

% Generalizing further to more general Tanner codes could allow to apply the flowering protocol on codes with linear time encoding.
% This could be the first step towards arithmetizing computations to codes on flowering-friendly graphs and creating a flowering-based SNARK.

\begin{credits}
% Ça ira seulement dans la version désanonymisée
\subsubsection{\ackname}
The authors deeply thank Tanguy Medevielle and Élina Roussel, with whom this work was initiated as the continuation of \cite{DMR25} that first defines the Flowering protocol.
The authors also thank Daniel Augot for his proofreadings and guidance and Pierre Loisel for his help regarding group theory and Cayley graphs.
The authors finally thank ChatGPT for its help to find relevant bibliography on expander graphs and to find spelling mistakes.

\subsubsection{\discintname}
The authors have no competing interests to declare that are
relevant to the content of this article.
\end{credits}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../CANS"
%%% End:


==> src/proof-soundness.tex <==
\subsection{Proof of soundness}

\begin{proposition}[Commit soundness]
  
\end{proposition}

\begin{proof}
  
\end{proof}

\begin{lemma}[Making events disjoints]
  
\end{lemma}

\begin{proposition}[Query soundness]
  
\end{proposition}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../CANS"
%%% End:


==> src/protocol-parameters.tex <==
\subsection{Flowering protocol parameters}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../CANS"
%%% End:

